Actuators \`A La Mode: Modal Actuations for Soft Body Locomotion

Traditional character animation specializes in characters with a rigidly articulated skeleton and a bipedal/quadripedal morphology. This assumption simplifies many aspects for designing physically based animations, like locomotion, but comes with the price of excluding characters of arbitrary deformable geometries. To remedy this, our framework makes use of a spatio-temporal actuation subspace built off of the natural vibration modes of the character geometry. The resulting actuation is coupled to a reduced fast soft body simulation, allowing us to formulate a locomotion optimization problem that is tractable for a wide variety of high resolution deformable characters.

==> 03_related_backup.tex <==


\section{Related Work}
%
\Otman{Otman's stupid redraft. People have done soft body controller in graphics, a bunch of different ways. Open loop, closed loop, trained with RL, genetic algorithms/gradient descent/or newton descent. 
The bottleneck in all these cases is always the same. The complexity of the simulation with the mesh resolution. 
Soft body simulation is a thing but has remained used so far mainly for passive simulation.
A few works make use of reduced or soft body modelling to perform trajectory optimization. The Pan/Manocha one, which focuses on trajectory optimization tasks, requiring lots of user guidance in the form of keyframes and constraints and the Liang one, which results in nonphysical actuation and has remained limited to low resolution geometries. 
}

\subsection{Soft Body Controllers}
Creating locomotion controllers for soft-body characters has a number of technical challenges.
%
The physical model used for simulation is often characterized by a large number of degrees of freedom, leading to bottlenecks during controller optimization.  
%
This in turn thwarts efforts in control which rely on simulation roll outs, while introducing additional difficulty in managing large observation and actuation spaces. 
%
A limited amount of previous work addresses constructing soft body controllers, with the significant majority modeling the full space of the character geometry.  Due to the increased complexity from using high resolution models, most only  animate simple 2D or coarse 3D characters \citet{coros2012deformablebodiesalive, jain2011modal, tan2012softbodylocomotion}.
%

Even with the use of simpler physics models and character geometries, 
\citet{bhatia2021evolution, lin2020softgym, huang2024dittogym,  hu2019difftaichi, rojas2021differentiable, min2019softcon} all report that training controllers for soft-body creatures with fewer than several thousand degrees of freedom can require hours, or even days, of training time, with simulations running much slower than real-time.


% SA: want to be careful about such generalizations, which aren't necessarily true...
%Regardless of what kind of controller you employ, the complexity of optimization for your controller is always bottlenecked by the simulation.
%Simulation time for soft body characters is always much more expensive than for rigid body characters, due to the explosion in the number of simulation degrees of freedom.

The large number of degrees of freedom (DOFs) required of soft-body simulations has motivated the development of reduced order models in order to improve simulation performance \cite{brandt2018hyperreducedpd, benchekroun2023fast, trusty2023subspacemfem}, with most of the prior work focusing on accelerating \textit{passive}  simulation. 
%
This work has been leveraged to accelerate trajectory optimization \cite{pan2018reducedtrajectoryoptimization}, it has seen limited use in accelerating general character controllers. 

While \citet{liang2023learningreducedordersoftrobotcontroller} also propose a reduced simulation, with a learned actuation within this reduced space, their resulting motions have been limited to extremely simple low resolution geometries. 
%
 Further we note that their approach introduces non-physical external torque artifacts upon actuation (see Figure~\ref{fig:frog-actuation-comparison}).

\subsection{Designing Character Musculature}

\Otman{Skeletal bodies have an easy musculature of joint torques, this is difficult to extend for soft bodies. 
Spring muscles have been proposed that can be used but require a user to place them correctly. Some people optimize for where to place these muscles/actuation structure, but this again has a large search space and works on very simple geometries. 
Yet another approach, Coros ,  Phace , Manocha and  propose a musculature whereby the input rest geometry of a tet mesh all change based on  rest geometry, a user-prescribed objectives, scan data, or a coarse cage. 
Our approach similarly encourages the shape towards a new rest-shape, but in our case, this rest shape is prescribed by natural vibrations of the character geometry.
}
Beyond fast simulation, an important step in designing controllers for a character lies in defining a viable musculoskelature for activating the physical system.

By far the most common method of constructing this structure for rigid articulated characters is through the use of joint torques applied at the intersection of adjacent bones \citet{yin2007simbicon, 
 xu2023adaptnet}. These joint torques are actuated directly, or indirectly through desired joint angles via PD controllers \cite{reda2020howenvironmentmattersforrl, tan2011stable}. 
%
Similar joint torques have been used to model soft-body characters whose motion is \textit{skeleton} driven \cite{libin2013skeletondrivensoftbodycontrol, kim2011direct, kim2011fast}, but this is does not generalize to arbitrary soft body characters where a skeleton is either not obvious or non-existent.

Instead of joint torques, \citet{geijtenbeek2013flexible} use biomechanically inspired muscles, resembling springs with adjustable rest lengths. 
%
This results in natural-looking motions, with the promise of less dependence on manually specified user parameters like joint torque limits.
%
Further, they ease the creation of contractile spring-like structures in deformable bodies \cite{rojas2021differentiable}.

Of course, the configuration and placement of muscles play an important contribution to the type of control that can be achieved.
%
\citet{lee2009biomechanicalmodellingupperbody, lee2014locomotion, lee2019scalable, saito2015computational, keller2023skintoskeleton} all propose highly detailed musculoskeletal models based on the real-world human anatomy.
%
However, as we explore different character morphologies, ``realistic'' anatomical models become ill-defined, and many methods rely on a user to manually design the placement of muscle fibers.
%
%
In the absence of an anatomical model, designers are left to their own devices, and often opt to draw muscles directly onto the character~\cite{tan2012softbodylocomotion, min2019softcon}. %themselves.

% can design three different types of muscles contractile muscles, radial muscles and . Then solves a trajectory optimization problem. Can draw contractive and bending muscles on character. Trains to actuate these muscles with a novel type of central pattern generator, modulated by DRL.

% \citet{liang2023learningreducedordersoftrobotcontroller} reduced simulation for simple characters, showing feedback control. The muscle structure is unspecified, and is instead learned by the controller itself. Expensive, but also unclear.

Alternatively, others shift the burden onto an optimization procedure to design the control actuation structure~\cite{lin2020softgym, bhatia2021evolution, ma2021diffaqua, liang2023learningreducedordersoftrobotcontroller}. 
%
The resulting optimization has a large search space, and has been shown to work best on very simple character geometries.

Another solution to designing character musculature lies in avoiding doing so altogether, instead reformulating the locomotion task as a trajectory optimization 
\cite{schulz2014deformablespacetimeconstraint,  pan2018reducedtrajectoryoptimization}. 
%
This shifts the burden on defining optimization objectives on the time-varying positions and additional objectives that keep the motion physical, usually requiring a  larger optimization problem.

\cite{jain2011modal} build controllers that only track the lower frequency modes of the simulation.
%

Finally,  \citet{coros2012deformablebodiesalive} propose a muscle actuation structure governed by the pose of a coarse approximating cage, which updates the target rest shape of the character, parameterized by the low dimensional DOFs of the cage. 
%
This work closely matches our own, with the key difference being that our target pose is parameterized by the elastic eigenfunctions of the shape, rather than a user-defined coarse cage.


\subsection{Motion Priors, Subspaces and References}
\Otman{They're key for creating natural motion in underspecified objectives. 
Many come from data, this tyle of controller has exploded with the rise of Deep Learning and its combination with Reinforcement Learning.
This data is great for specific character morphologies where data is ample, but for soft bodies this motion data is much scarcer. 
One way to proceed without motion data is to impose stricter objectives (Manocha, Hees, YuPeriodic) that guide  .
Others instead change the actuation/control space itself, to reflect properties of the motion, such as low-dimensinoal info from synthetic data (motor babble).
In particular some have imbued their actuation space to be periodic  (Manocha, Starke, Min, CPG works), an assumption with long-standing roots in biomechanical modelling of animal gaits.
while others and energy efficiency (Kry, Nunes, Jain)
, resulting in a motion that is defined as lying in that space. 
}
Reference signals and motion priors that influence the controller are often used
to specify characteristics of the desired motion, for example to 
make a behavior appear more humanlike or natural.  
%
With the rise of deep learning, its combination with reinforcement learning has enriched our ability to use human motion to great success in this capacity.
For example ~\citet{peng2018deepmimic} employ reinforcement learning to successfully imitate reference motion to closely mimick a variety of human behaviors.
%

Many alternatives have been introduced for inserting motion data into DRL frameworks.  For example, some encode motion data in latent spaces~\cite{holden2015learningmotionmanifoldscnn, holden2020learnedmotionmatching, bergamin2019DreCon}.Others employ discriminants to differentiate good motion from bad using reference motion to compare with simulated motion~\cite{peng2021amp,iccgan}.  Meanwhile, others extract
data with specific cyclic properties, and imbue the network architecture itself with this property
\cite{holden2017phasefunctionnn, starke2023deepphase}. A survey of these and more appears here~\cite{DRLSurvey}.

In contrast, in soft body control, reference motion is not usually readily available.  Thus, alternatives for generating control inputs are 
often necessary; a number of alternatives have been proposed to support controllers without recorded data. 
%including modal decomposition and 
%other approaches.
%modal analysis has seen some attention in several works.
%

Some report success without reference motion, through stricter objectives and training routines. 
%
\citet{heess2017emergence} turn to a more rigorous training routine to fill the hole, observing that training a controller on a diverse set of environments leads to much more robust rigid-body controllers that can satisfy user defined objectives, albeit with some undesired jittery motion.
\citet{yu2018LearningSymmetricLocomotion} make use of both symmetry and periodicity, combining these principles with curriculum learning to generate locomotion controllers with no motion data whatsoever.

Others turn to energy efficiency,  \citet{kry2009modallocomotion} and \citet{ nunes2012naturalvibrationslocomotion} show that that the natural vibrations of articulated characters can be used to to generate locomotion animations and simple controllers, while 
%
\citet{ranganath2021motorbabble} generate synthetic motion data for articulated characters, and derive control signals using Principal Component Analysis (PCA) applied to the synthetic data.
%
They then train a DRL agent to build control policies from this reduced control space to animate characters with varying morphologies.

Further, Central Pattern Generators (CPG) \cite{guertin2009mammalian} offer a simple model for periodic motion control signals that are propagated across the character. 
%
This model has been leveraged for motion control as it requires only a handful of periodic and spatial parameters, such as propagation speed frequency, to generate motion\cite{min2019softcon, tan2011articulated}.



==> 040_method.tex <==
\section{Method Overview}
%
Our \textit{Modal Muscles} are comprised of two \textit{separate} subspaces, one for control and one for simulation, and an actuation structure that interfaces the two. 

%
We derive the control subspace from Modal Analysis \cite{pentlandwilliams1989goodvibrations}, with the notion that characters accomplish tasks in an energy efficient manner.
%
This assumption allows our controller to find locomotions with semantically meaningful deformations, such as the bat flapping its wings to move forward in \reffig{bat-modal-actuation}. 
%
Because our characters may be meshes of arbitrarily high resolution, we also adopt a Skinning Eigenmodes \cite{benchekroun2023fast} simulation subspace, which allows us to perform our many simulation evaluations without scaling with the character complexity.
%
Finally, we adopt the plasticity-based muscle actuator from \cite{coros2012deformablebodiesalive, alecandru-eugen2017phace}, which guides the simulated character towards a target shape in our control subspace. 

% The first 
% \Otman{Make sure to clarify that there are two reduced models... one for control actuation and one for simulation, and they're separate but they are related.}
% \Otman{Method overview is very  matter of fact and doesn't take into account any philosophy of design. Try to highlight that we care about energy efficiency more, give some intuition for why a reduced order model would be reasonable. Give some intuition for what the muscle model means philosophically.}


% % Our method constructs a geometric motion subspace based off the energetically optimal vibration modes of the character. 
% % %
% % This prior is entirely determined by the geometry of the character, requiring no motion data whatsoever.
% % %
% % This prior is used by the controller to specify target shapes our character, from an energetic standpoint, prefers to take.


% %
% We then leverage this prior to define a "muscle" actuation, which provides a force over the whole character guiding it towards the target shape within our motion subspace. The motion subspace, combined with our muscle model, allow us to drastically reduce the space of controls available to the control optimization. 

% %
% In order to fully capitalize on the reduced dimension of our motion subspace, we combine our muscle model with a reduced-space simulation, which allows us to generate controllers for characters of arbitrarily high geometric resolution.

% \Otman{Appendix should show how we compute $a_{min}$ and $a_{max}$}

\input{041_motion_prior}

\input{042_muscle_model}

\input{043_reduced_simulation}

\input{044_projective_solver}

==> 041_motion_prior.tex <==
\subsection{Modal Control Subspace}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/seal-control-modes.pdf}
    \timestamp{\tsSealControlModes}
    \caption{The first 5 non-rigid elastic vibration modes of a seal, corresponding to reasonable low-energy motions one could expect to see from a seal.}
    \label{fig:seal-control-modes}
\end{figure}


Without access to motion data, our guiding principle becomes energy efficiency.  
%
Taking inspiration from the shape analysis literature \cite{levy2006eigenfunctions, pentlandwilliams1989goodvibrations}, we construct a motion subspace based off of the energetically optimal vibration modes of the character.
%
While these vibration modes have been used by many prior works for reducing \textit{passive} simulations, we show that they also form a strong subspace for \textit{active} motion control tasks.
%

We perform modal analysis of the elastic energy Hessian $\H = \frac{\partial  E}{\partial \x^2} \in \Rn{3n \times 3n}$,

\begin{align}
    \H \D = \M \D  \boldsymbol{\Lambda},
    \label{eq:motion-prior-spatial}
\end{align}
and obtain $\D \in \Rn{3n \times m}$ the eigenvectors that form the spatial basis for our motion subspace.
%
Above, $\M \in \Rn{3n \times 3n}$ is the block diagonal vector-mass matrix. $\boldsymbol{\Lambda}$ is a diagonal matrix of eigenvalues. 
%
These eigenvectors correspond to motions that incur \textit{least} amount of elastic energy and are visualized in \reffig{seal-control-modes} for a seal. 
%
We refer to each of these eigenvectors as the \textit{control modes} of the character.

%
Deformed positions $\d \in \Rn{3n}$ in this basis of control modes can compactly be represented by a low dimensional time-varying actuation vector $\a(t) \in \Rn{m_s}$ (with $m_s$ being the number of control modes) as well as the rest geometry $\x_0 \in \Rn{3n}$,
\begin{align}
    \d = \begin{bmatrix} \D \quad  \x_0 \end{bmatrix} 
    \begin{bmatrix}
        \a(t)  \\
        1
    \end{bmatrix} = \bar{\D} \bar{\a}(t).
    \label{eq:target-shape}
\end{align}
Where the $\bar{\mathrm{bar}}$ denotes a homogeneous expression of this control space $\bar{\D} = [\D \; \x_0] \in \Rn{3n \times (m+1)}$ and $\bar{\a} = [\a(t) \; 1]^T  \in \Rn{m+1}$, which we employ to simplify future expressions.
%
Taking inspiration from energy efficiency, and with the intuition that many of the locomotion gaits we observe are smooth and periodic, we form a temporal subspace via a sum of $m_t$ sinusoids,
\begin{align}
    \a_i(t) =  \sum_j^{m_t} \boldsymbol{A}_{ij} \mathrm{sin}\left(2 \pi  (\frac{t} {\T_{ij}} + \boldsymbol{\theta}_{ij} )\right).
\end{align}
%
where $\A_{ij}, \T_{ij}, \boldsymbol{\theta}_{ij}$ are the amplitude, period and phase shift for each control mode $i$ and sinusoidal function $j$. 
%
These quantities form the degrees of freedom (DOFs) for our controller, $\p = [\A \;\T  \;\boldsymbol{\theta}]^T \in \Rn{3 m_s \times m_t}$.



% \begin{figure}
%     \centering
%     \includegrathetacs[width=0.5\linewidth]{images/white.png}
%     \caption{Energy landscape as we vary the first control mode's amplitude, setting all other optimization parameters fixed. We show lines of different colors for varying the number of control modes with $m_s$, while keeping $m_t$ fixed to one. By decreasing $m_s$, the optimization problem becomes smoother and smoother.}
%     \label{fig:energy-landscape-reduction}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/white.png}
%     \caption{ Many degrees of freedom can lead to an unnatural, jittery motion, restricting our optimization problem within our motion prior recovers smoother, more realistic gaits.}
%     \label{fig:jittery-motion}
% \end{figure}



==> 042_muscle_model.tex <==
\subsection{Muscle Model}\label{sec:muscle_model}
With our motion subspace in  hand, we derive a plasticity-based muscle actuator like \citet{coros2012deformablebodiesalive}, that encourages 
the character to take on a target shape in our control subspace $\a$ via \refeq{target-shape},

\begin{align}
    \mathcal{E}_m(\x, \a) &= \mathcal{\psi}(\x)  + \mathcal{\phi}(\x, \a) \\
    \mathcal{\psi}(\x) &= \int_{\mathcal{N}} \min_{\R \in \mathcal{SO}(3)}
      \mu  ||\F(\x) - \R ||^2_Fd\x \\
    \mathcal{\phi}(\x, \a) &= \int_{\mathcal{N}} \min_{\bOmega \in \mathcal{SO}(3)}
      \gamma || \F(\x) - \boldsymbol{\Omega} \Y(\a) ||^2_F  d\x,
    \label{eq:continuous-muscle-energy}
\end{align}
where $\F(\x)$ corresponds to the deformation Jacobian of the material, while $\Y(\a)$ is a target deformation Jacobian obtained from the actuation $\a$.
%
Our muscle energy is comprised of a passive term  $\mathcal{\psi}$ that penalizes deformation of any kind (which is just the familiar ARAP elastic material model  \cite{olgasorkine2007arap, kim2022dynamicdeformables}), and an active term $ \mathcal{\phi}$ that encourages the deformation field $\F$ to match the one described by the target $\Y(\a)$.
%

Increasing $\mu$ relative to $\gamma$ allows us to counteract potentially unnatural target motions that may arise out of over-actuating our linear control modes, as shown in \reffig{bat-modal-actuation}.
%

We focus the remainder of our discussion on the less common $\textit{active}$ term $\phi$.
%
The locally defined best fit rotation matrix $\boldsymbol{\Omega}$ filters out rotations from our measure of muscle actuation;
%
The actuation $\a$ should lead to the same motion regardless of how the simulated shape $\F(\x)$, and the control target shape $\Y(\a)$ are oriented.
%
This also ensures our muscle actuation conserves angular momentum, which is not the case for the force-based actuation model of \citet{liang2023learningreducedordersoftrobotcontroller} which can introduce spurious linear and angular forces as shown in \reffig{frog-actuation-comparison}.
%

%
% Formulating this change in rest state as an objective additionally allows us to carry it through to our projective dynamics solver in \ref{sec:local-global-solver}, saving us many costly matrix recomputations that come from changing the rest state.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/bat_modal_actuation.pdf}
    \timestamp{\tsBatActuation}
    \caption{The active component of our muscle energy attempts to match a target modal displacement, even if that displacement incurs unnatural volume gains. The passive component of our muscle energy penalizes excessive deformation, and mitigates this issue. Their combination allows the bat to naturally flap its wings. }
    \label{fig:bat-modal-actuation}
\end{figure}




\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/actuation_comparison.pdf}
    \timestamp{}
    \caption{Allowing a force actuation that directly spans the first few elastic vibration modes, like \cite{liang2023learningreducedordersoftrobotcontroller}, allows for the character to control non-physical external forces, leading to spurious rotations and translations. }
    \label{fig:frog-actuation-comparison}
\end{figure}


==> 043_reduced_simulation.tex <==
\subsection{Reduced Simulation}\label{sec:reduced_simulation}
Less degrees of freedom usually also comes with the promise of a faster solution to the optimization problem.
%
However, optimizing for a character controller typically requires many forward evaluations of the simulation itself, with many state of the art controllers requiring hundreds of thousands of simulation timesteps \cite{tan2011articulated, min2019softcon, reda2020howenvironmentmattersforrl}.
%
Because the simulation scales in complexity with the mesh, the cost of the simulation ends up being the main bottleneck of the control optimization process.
%
% F
% %
% Obtaining such a controller for the highly detailed deformable bodies we care about quickly becomes untractable.  \Otman{WHy do we care about them? Where do establish what kind of geometry we care about.}
% %
In order to make the control optimization tractable for the high resolution geometries we have in mind, we decouple the simulation step from the resolution of the mesh using Reduced Order Modelling \cite{barbicjames2005realtimestvk}.
%

We start with the variational problem for soft body simulation, discretizing the kinetic energy and the muscle energy from \refeq{continuous-muscle-energy} with linear finite elements.
%
Every timestep the simulation solves for a set of per-vertex positions $\x \in \Rn{3n}$ that minimize the system's physical energy,
\begin{align}
     \argmin_{\x}& {\frac{1}{2h^2}|| \x - \y ||^2_{\M}} +  \Psi(\x) + \Phi(\x, \a)  \\
     \Psi(\x) =& \sum_t^{|\mathcal{T}|} \min_{\R_t \in \mathcal{SO}(3)}
  \mu_t  ||\F_t - \R_t ||^2_F, \\
  \Phi(\x, \a) =&  \sum_t^{|\mathcal{T}|} \min_{\bOmega_t \in \mathcal{SO}(3)}
   \gamma_t || \F_t - \bOmega_t \Y_t ||^2_F
\end{align}
with $h$ being the simulation timestep, $\y = 2 \x_{curr}  - \x_{prev} \in \Rn{3n}$ is an inertial displacement, $\Psi$ and $\Phi$ are the passive and active muscle energies respectively, which are computed as a sum of per tetrahedron energy densities over all tetrahedra $|\mathcal{T}|$.

\subsubsection{Skinning Eigenmode Subspace}
We reduce our positional degrees of freedom $\x$ with a linear Skinning Eigenmode subspace \cite{benchekroun2023fast},
\begin{align}
 \x = \B(\W) \z   
\end{align}
where $\z \in \Rn{r}$ are the reduced space vertex positions. 

%
$\B(\W) \in \Rn{3n \times r}$ is a subspace matrix, parameterized by a set of Linear Blend Skinning weights $\W \in \Rn{m}$, with $r=\mathrm{dim}(\mathrm{dim} +1)m= 12m$.
%
We obtain these weights from a modal analysis on the elastic energy Laplacian, $\L = \frac{\partial^2 E}{\partial \x_x^2} + \frac{\partial^2 E}{\partial \x_y^2} + \frac{\partial^2 E}{\partial \x_z^2} \in \Rn{n \times n}$,
\begin{align}
\L \W &= \M \W \boldsymbol{\Lambda}.   
\label{eq:skinning_eigenmodes_gevp}
\end{align}
%
$\B$ is then constructed from $\W$ via the equation:
\begin{align}
\B &= \I_3 \otimes ( \W \otimes \boldsymbol{1}_4^T ) \odot (   \boldsymbol{1}_m^T  \otimes [\X \; \boldsymbol{1}_n] ).
\label{eq:lbs_jacobian}
\end{align}

\subsubsection{Clustering $\bOmega_t$}
However, despite achieving a reduction from our position degrees of freedom $\x$, our non-linear rotation term  $\bOmega_t$ introduces another problem.
%
Because this term needs to be solved for for each tetrahedron, every simulation step, our simulation is once again tied to the full resolution of the mesh.
%
To resolve this, we derive a novel clustering scheme for our active muscle energy, providing a reduction from the full number of tetrahedra $|\mathcal{T}|$.

Specifically, we allow for multiple tetrahedra to share the same rotation matrix $\bOmega_{c(t)}$, where $c(t) \in |\mathcal{C}|$ identifies the cluster $c$, in the set of clusters $|\mathcal{C}|$ to which tetrahedron $t$ belongs. 
%
Our novel approximation for the active term of our muscle energy becomes,
\begin{align}
\begin{split}
         \Phi(\x, \a) \approx  \tilde{\Phi}(\x, \a) =  \min_{ \bOmega_c}  \sum_t^{|\mathcal{T}|} 
    \gamma_t || \F_t - \bOmega_{c(t)} \Y_t ||^2_F  \\
     s.t. \; \bOmega_c \in \mathcal{SO}(3) \; \forall{c} \in |\mathcal{C}|.
    \label{eq:clustered-active-term}    
\end{split}
\end{align}
We prove in \refapp{optimal-clustered-rotations} that the optimal clustered rotation $\Omega_c(t)$ minimizing the objective above can be found via a polar decomposition of the $\gamma$-weighed sum of the covariance matrix $\F_t \Y_t^T$,
\begin{align}
    \bOmega_c  =   \mathrm{polar} \left( \H_c \right) = \mathrm{polar} \left( \sum_t^{|\mathcal{T}(c)|} \gamma_t \F_t \Y_t^T \right), 
    \label{eq:optimal_rotations}
\end{align}
Where $\  \mathrm{polar}(\H_c)$ is a function performing polar decomposition on $\H_c$ in order to achieve its rotational component $\bOmega_c(t)$. 
%

While evaluating this term once again involves a per-tet sum, we notice that this sum is a bilinear form in our two low-dimensional time-varying quantities, $\z$ and $\bar{\a}$. 
%
With this intuition, we show in \refapp{tensor-precomp} that by precomputing the appropriate tensor we can efficiently evaluate this sum at run-time in a manner scaling only in complexity with our small $\z$ and $\bar{\a}$.

\begin{align}
\H_{cij} &=    \mathcal{H}_{cijuv} z_u \bar{a}_v .
\label{eq:tensor_covariance_matrix}
\end{align}

Above, we have introduced the tensor $\mathcal{H} \in \Rn{|\mathcal{C}|  \times 3 \times 3 \times r \times(m_s + 1)}$, which we derive in \refapp{tensor-precomp}, that when multiplied against $\z$ and $\bar{\a}$ (in homogeneous coordinates) computes our per-cluster covariance matrix $\H \in \Rn{|\mathcal{C}| \times 3 \times 3}$.
%
Note that evaluating $\H_c$ every stimulation step via this tensor product only requires operations that scale with the number of clusters $|\mathcal{C}|$, the dimension of our reduced positional DOFS $\z$, and the size of our control actuation $\bar{\a}$.

%
% Ensuring these clustered rotation matrices remain the minimizers of the energy is crucial in preserving global rotation invariance, and in turn guarantees that the muscle forces are momentum conserving.

To derive the clustered approximating energy for the passive muscle term $\tilde{\Psi}$, along with its efficient tensorial expression for $\R_{c(t)}$, one only needs to set  $\Y_t$ in \refeq{clustered-active-term} to the identity and swap $\gamma_t$ for $\mu_t$. This ends up giving the same clustered ARAP energy as \citet{jacobson2012fast}.

%
Finally, after plugging in the positional subspace $\x = \B \z$, and swapping out the passive and elastic energies $\Psi, \Phi$ for their clustered approximations $\tilde \Psi, \tilde \Phi$, the reduced-space optimization problem that needs to be solved every simulation timestep becomes:
\begin{align}
              \argmin_{\z} \frac{1}{2h^2}|| \z - \q ||^2_{\N} + \tilde{\Psi}(\z) + \tilde{\Phi}(\z, \a),  
              \label{eq:reduced-clustered-optimization-problem}
\end{align}
with $\q = \B \y \in \Rn{r} $ being our reduced inertial positions and $\N =\B^T \M \B  \in \Rn{r \times r}$  being the reduced space mass matrix. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/active-clusters.pdf}
    \caption{ Decreasing the number of active clusters accelerates the speed at which our simulated shape matches the target descirbed by the control signal. }
    \label{fig:jittery-motion}
\end{figure}


==> 044_projective_solver.tex <==
\subsubsection{Local Global Solver}
\label{sec:local-global-solver}
We make use of a local global solver to solve our reduced physics optimization problem.
%
The \textit{local} step first holds $\z$ fixed and optimizes for $\R_t$ and $\bOmega_t$ using \refeq{tensor_covariance_matrix} and \refeq{optimal_rotations}.

%
Then, the \textit{global} step holds $\R_t$ and $\bOmega_t$ fixed, optimizing for $\z$. This is resolved using a linear solve we derive in \refapp{global-step-derivation},
\begin{align}
    \Q & \z = \f ,
    \label{eq:local-global-system}
\end{align} 
with $\f \in \Rn{r} $ and  $\Q \in \Rn{r \times r} $ given by,
\begin{align}
    \Q &= \Q^{\M} + \Q^{\Psi} + \Q^{\Phi}, \\
    \f &=  \f_{\M}(\z, \z_{vel})+ \f_{\Psi}(\R) + \f_{\Phi}(\bOmega) + \f_c(\z). 
\end{align} 

The system matrix $\Q$ is a sum of an inertial Hessian $\Q^{\M}$, a passive elastic energy Hessian $\Q^{\Psi}$, and an active elastic energy Hessian $\Q^{\Phi}$.
%
It's important to note that all contributions to the system matrix are constant, computed once at rest, and never recomputed again.
%
This allows us to precompute a Cholesky decomposition for the solve \textit{once}, and continuously reuse it all the way throughout the \textit{entire} controller training pipeline.

%
The right hand side to the system in \refeq{local-global-system} $\f$ is a sum of inertial forces $\f^{\M}$, passive elastic forces $f^{\Psi}(\R)$, active elastic forces $f^{\Phi}(\bOmega)$, and contact forces $\f^c(\z)$.
%

The contact forces are found such that the resulting simulation after the global step solve in \ref{eq:local-global-system} satisfies our no rebound, zero-slip condition.
%
To maintain reduced complexity, we enforce this condition and do collision checks on a pre-prescribed subset of possible contact points, which we obtain via farthest point sampling on the surface of the mesh.






\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/tardigrade-subspace.pdf}
    \caption{ We visualize the three simulation subspace parameters, namely 4 Skinning Eigenmodes, 10 passive muscle clusters and 30 contact sample points. }
    \label{fig:jittery-motion}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/subspace_timings.pdf}
    \caption{ Timings of 200 simulation steps as we vary three simulation subspace parameters of our reduced simulation, the number of skinning eigenmodes, contact samples, and passive muscle clusters.}
    \label{fig:jittery-motion}
\end{figure}



==> 05_implementation.tex <==
% \section{Implementation}
% \label{sec:implementation}

% We implement our entire algorithm in Python, using $\texttt{numpy}$ and $\texttt{scipy}$ for our simulation step.

\begin{algorithm}[h]
   \caption{Performs one simulation step of our Modal Muscles reduced space controlled simulation, taking as input current reduced space positions $\z \in \Rn{r}$, inertial positions $\q \in \Rn{r}$ and a control signal $\a \in \Rn{m}$. \label{alg:environmentStep}}
 \SetKwFunction{FsimulationStep}{simulationStep}
  \SetKwProg{Fn}{Function}{:}{}
\Fn{\FsimulationStep{$\z, \q, \a$}}{
\While{$\mathrm{not\, converged}$}
{ 
    $ \f^p \gets \mathrm{passiveForce}(\z, \q)$ \\
    $\f^a \gets \mathrm{activeForce}(\z, \a) $ \\ 
    $\f^c \gets \mathrm{contactForce}(\a, \f^a + \f^p)$\\
    $ \z \gets \Q^{-1} (\f^p + \f^c + \f^c )$ \\ 
}
\KwRet $\z$
}
\end{algorithm}


% \begin{algorithm}[h]
%    \caption{. \label{alg:passiveForce}}
%  \SetKwFunction{FpassiveForce}{passiveForce}
%   \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FpassiveForce{$\z, \q$}}{
% \While{$\mathrm{not\, converged}$}
% { 
% }
% \KwRet $\f^p$
% }
% \end{algorithm}


\begin{algorithm}[h]
   \caption{. \label{alg:activeForce}}
 \SetKwFunction{FactiveForce}{activeForce}
  \SetKwProg{Fn}{Function}{:}{}
\Fn{\FactiveForce{$\z, \a$}}{
{   
$\bar{\a} \gets \begin{bmatrix}\a \\ 1\end{bmatrix}$ \\
    $\H \gets (\mathcal{H}:\z):\bar{\a}$\\
$\bOmega \gets \mathrm{polar}(\H)$ \\
$\f^a \gets (\mathcal{O}:\bOmega):\bar{\a} $ \\
}
\KwRet $\f^a$
}
\end{algorithm}

\begin{algorithm}[h]
   \caption{. \label{alg:contactForce}}
 \SetKwFunction{FcontactForce}{contactForce}
  \SetKwProg{Fn}{Function}{:}{}
\Fn{\FcontactForce{$\z, \f$}}{
{   
$\c \gets \K \z  $ \\
$ \mathbf{cI}_N, \mathbf{cI}_T \gets \mathrm{interpenetratingIndeces}(\c)$ \\ 
$\L \gets \K[\mathbf{cI}, :] \Q^{-1} $ \\
$\b \gets \K[\mathbf{cI}, :] \z - \L \f$ \\ 
$ \f^c \gets \mathrm{pseudoInverse}(\L, \b)$
}
\KwRet $\f^a$
}
\end{algorithm}






% \section{Implementation}


==> 08_acknowledgements.tex <==
\begin{acks}

\end{acks}

==> related_backup_victor.tex <==
\section{Method Overview}
Our goal is to derive an actuation for deformable characters that generates motion satisfying certain objectives, while remaining physically plausible.
%
We  cast this as a controller optimization problem \cite{coros2012deformablebodiesalive},
%
\begin{align}
    \min_{ \d(t)}\quad & J(\x(t)) \label{eq:objective_full_space}, \\
    \begin{split}
        \text{s.t.} \quad  \x|_t = \argmin_{\x}   \quad &  E(\x,  \d|_t), \forall t \in [t_0, t_1] \label{eq:full_space_sim}\\
        % \text{s.t.} \quad & \C(\x(t)) \leq \boldsymbol{0} 
    \end{split}
\end{align}
where we are solving for a time-varying actuation $\d(t) \in \Rn{3n}$ that corresponds to the target shape our character should take.
%
$J(\x(t))$ is a task-specific objective on the vertex positions $\x(t) \in \Rn{3n}$ that rewards desired motions (e.g for a locomotion task, it can reward motion of the center of mass along a target direction).

%
The constraint \refeq{full_space_sim} ensures the resulting motion abides the laws of soft-body physics with contact; The vertex positions at any point in time $\x|_t \in \Rn{3n}$ must be the minimizers of the total energy $E(\x|_t, \d|_t)$ of the physical system.
%
This physical energy can be split into two components,  
\begin{align}
E(\x, \d) = E_p(\x) + E_a(\x, \d),   
\end{align}
a passive component $E_p(\x)$ that captures motion according to inertia, external forces, and elastic forces, and an active component $E_a(\x, \d)$ that encourages the elastic body to take on the shape of $\d$.
%

On top of being non-linear in both $\x(t)$ and $\d(t)$, \refeq{objective_full_space} becomes especially difficult to solve for high resolution characters because the problem scales in complexity with the increased dimensionality of $\x(t)$ and $\d(t)$.
%
The sour combination of high non-linearity and high dimensionality makes solving this problem an extremely slow process prone to large null spaces.


Our solution to these problems is to introduce an actuation subspace for $\d$ based off of the natural elastic vibration modes of the character \cite{pentlandwilliams1989goodvibrations}. 
%fOur 
We combine this reduction with a separate simulation subspace for $\x$, built off Skinning Eigenmodes \cite{benchekroun2023fast}. 
%
The separation of these two subspaces allow us to independantly tailor each one to their own specific tasks, actuation and simulation, which have different desiderata.

%
We then show how to carry out simulation in these reduced spaces while remaining independent from the resolution of the mesh.
%
Our reduced-space framework allows us to quickly evaluate simulations of arbitrarily high resolution characters.

This speedup in simulation evaluation lends itself well to the use of a CMAES \cite{hansen2006cma} optimizer in order to solve our control optimization \refeq{objective_full_space}. 
%
This derivative-free genetic algorithm iteratively samples populations of $\d(t)$, which are used to drive multiple simulations. 
%
The resulting objective $J$ is measured for each simulation, and is used by CMAES to inform the collection of a next, more optimal generation of $\d(t)$.
%
The process is repeated until convergence, or until a maximum number of iterations are achieved.



% comprised of four terms
% \begin{align}
%     E(\x, \d) = \underbrace{E^K(\x)  + E^{\Psi}(\x) + E^c(\x)}_{\mathbf{passive}} + \underbrace{E^{\Phi}(\x, \d)}_{\mathbf{active}}
% \end{align}


%

% \begin{align}
%     \mathbf{C}(\x(t), \d(t)) = \0 \; \implies  \; 
%     \x(t) = \argmin_{\x(t)}  \quad  E(\x(t), \d(t)).
% \end{align}


% of the are the minimizer of a soft body simulation energy $E$ guided by the control signal $\d(t) \in \Rn{3n}$ at time $t$, represented as a set of target vertex locations.
%
% We optimize the control signal $\d$ with evolutionary algorithms (e.g., CMAES \derek{citation?}) such that the character $\x$ guided by $\d$ minimize the objective function $\mathbf{J}$.
% % Our goal is to optimize the control signal $\d$ so that the character $\x$ guided by $\d$ minimize the objective function $\mathbf{J}$.

% However, this optimization problem is highly non-linear in $\d$. For high resolution characters, solving \refeq{objective_full_space} in the full space $\Rn{3n}$ often leads to intractable computation costs because evolutionary methods require many simulation evaluations to optimize the objective. In addition, optimizing in such a non-linear high-dimensional space is prone to bad local minima.
% %
% Our primary contribution is to reduce the control space from $\d \in \Rn{3n}$ to a \emph{control subspace} $\a in \Rn{r}$, we called \emph{Modal Muscles}, to greatly reduce the degrees of freedom in the optimization $r << 3n$. 
% %
% Our modal muscles help avoid bad local minima and achieve plausible locomotion for a variety of deformable characters (see \reffig{teaser}).
% %
% In addition, we adopt the method by \citet{benchekroun2023fast} and use the subspace simulation method to reduce $\x \in \Rn{3n}$ to $\z \in \Rn{r}$, which allows us to efficiently perform simulation evaluations $\argmin_{\x}  E$ without scaling with the character complexity.

% Combining our modal muscles $\a$ and the simulation subspace $\z$, our reduced optimization problem has the following formulation
%
% \begin{align}\label{eq:objective_subspace}
%     \min_{\a}\quad &\mathbf{J}(\z) \\
%     \text{s.t.} \quad &\z = \argmin_{\z}  E(\z, \a(t)) 
% \end{align}
% %
% where all the objective $\mathbf{J}$ and the energies $E$ are all defined in the reduced space $\z, \a$.
% %
% In \derek{cite section}, we discuss the construction of our modal muscles to reduce the ... \derek{finish up this part when we update the rest of the section.}

% \subsection{Modal Muscles Control Subspace}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/seal-control-modes.pdf}
%     \timestamp{\tsSealControlModes}
%     \caption{The first 5 non-rigid elastic vibration modes of a seal, corresponding to reasonable low-energy motions one could expect to see from a seal.}
%     \label{fig:seal-control-modes}
% \end{figure}
% %
% Our input can be an arbitrary (realistic or fantasy) deformable character. This implies that the construction of our modal muscles cannot rely on motion data. Our guiding principle thus becomes constructing a control subspace that is energy efficient. 

% Taking inspiration from the shape analysis literature \cite{levy2006eigenfunctions, pentlandwilliams1989goodvibrations}, we construct our subspace based off of the energetically optimal vibration modes of the character.
% %
% While these vibration modes have been used by many prior works for accelerating simulations \derek{add citations}, we show that they also form an effective subspace for controlling characters.

% Vibration modes are the solutions to the eigenvalue problem of the elastic energy Hessian $\H = \in \Rn{3n \times 3n}$
% %
% \begin{align}
%     \H \D = \M \D  \boldsymbol{\Lambda},
%     \label{eq:motion-prior-spatial}
% \end{align}
% %
% where $\M \in \Rn{3n \times 3n}$ denotes the block diagonal vector-mass matrix, $\boldsymbol{\Lambda}$ is a diagonal matrix of eigenvalues, and $\D \in \Rn{3n \times m}$ is a collection of eigenvectors.
% %
% These eigenvectors $\D$ correspond to motions that incur the \textit{least} amount of elastic energy (see \reffig{seal-control-modes}).
% %
% Our model muscles (control subspace) refer to the combination of these eigenvectors of the character.

% %
% Given these eigenbases $\D$, the target vertex positions $\d \in \Rn{3n}$ from the controller can be compactly represented by a low dimensional time-varying actuation vector $\a(t) \in \Rn{m_s}$ (with $m_s$ being the number of control modes) as well as the rest geometry $\x_0 \in \Rn{3n}$,
% %
% \begin{align}
%     \d = \begin{bmatrix} \D \quad  \x_0 \end{bmatrix} 
%     \begin{bmatrix}
%         \a(t)  \\
%         1
%     \end{bmatrix} = \bar{\D} \bar{\a}(t).
%     \label{eq:target-shape}
% \end{align}
% %
% Where the $\bar{\mathrm{bar}}$ denotes a homogeneous expression of this control space $\bar{\D} = [\D \; \x_0] \in \Rn{3n \times (m+1)}$ and $\bar{\a} = [\a(t) \; 1]^T  \in \Rn{m+1}$, which we employ to simplify future expressions.

% \subsection{Skinning Eigenmodes Simulation Subspace}
% %
% The natural vibration modes enable us to define control signals $\d$ in a reduced subspace $\a$ (\refeq{target-shape}).
% %
% The second reduction is to further reduce the degrees of freedom in simulation $\x$ to a lower dimensional subspace $\z$.

% For the simulation subspace, we use the linear Skinning Eigenmode subspace by \citet{benchekroun2023fast},
% %
% \begin{align}
%  \x = \B(\W) \z   
% \end{align}
% %
% where $\z \in \Rn{r}$ are the reduced space vertex positions, and $\B(\W) \in \Rn{3n \times r}$ is a subspace matrix, parameterized by a set of Linear Blend Skinning weights $\W \in \Rn{m}$, with $r=\mathrm{dim}(\mathrm{dim} +1)m= 12m$.

% \citet{benchekroun2023fast} obtain these weights from a modal analysis on the elastic energy Laplacian, $\L = \frac{\partial^2 E}{\partial \x_x^2} + \frac{\partial^2 E}{\partial \x_y^2} + \frac{\partial^2 E}{\partial \x_z^2} \in \Rn{n \times n}$,
% %
% \begin{align}
%     \L \W &= \M \W \boldsymbol{\Lambda},
%     \label{eq:skinning_eigenmodes_gevp}
% \end{align}
% %
% where $\B$ is constructed from $\W$ via:
% %
% \begin{align}
%     \B &= \I_3 \otimes ( \W \otimes \boldsymbol{1}_4^T ) \odot (   \boldsymbol{1}_m^T  \otimes [\X \; \boldsymbol{1}_n] ).
%     \label{eq:lbs_jacobian}
% \end{align}
% %



% \subsection{Reduced Muscle Energy}
% % \derek{not sure whether there is a better name for "control energy"? Previously, you name it active term, but I feel we can try to be more precise and intuitive in describing what this energy does.}
% Our muscle energy $\Phi$ (\refeq{objective_full_space}) encourages the vertices $\x$ of a character to match the target locations $\d$ produced by our modal muscles. 
% %
% More precisely, we define the muscle energy is the squared difference between the deformation Jacobians
% %
% \begin{align}
%     \Phi(\x, \d) &= \sum_t^{|\mathcal{T}|} \min_{\bOmega_t \in \mathcal{SO}(3)}
%       \gamma_t || \F_t(\x) - \bOmega_t \Y_t(\d) ||^2_F 
%     \label{eq:continuous-muscle-energy}
% \end{align}
% %
% where $\F_t$ corresponds to the deformation Jacobian of a tetrahedron $t$ defined on character vertices $\x$, $\Y_t$ is the deformation Jacobian derived from the target vertex locations $\d$ output from the controller, and  $\bOmega_t \in \mathcal{SO}(3)$ is the best fitted rotation to factor out rigid transformation.

% However, this energy is defined on the full space $\x, \d \in \Rn{3n}$ and may lead to expensive evaluations on high resolution meshes. 


% \subsection{Reduced Simulation}
% \derek{very similar to the old version that talks about the arap term and the kinetic term}

% \derek{I guess we can add a summary that re-write our \refeq{objective_subspace} with all the terms (in the reduced space) here.}

% \paragraph{Implementation Details}
% \derek{I feel talking about $\p$ here breaks the flow quite a lot. This is because the rest of the derivation is on $\a$, instead of $\p$. Maybe we should move it to "implementation details" at the end of the section}
% As many real-world locomotion gaits are smooth and periodic, we further parameterize $\a(t)$ via a sum of $m_t$ sinusoids,
% %
% \begin{align}
%     \a_i(t) =  \sum_j^{m_t} \boldsymbol{A}_{ij} \mathrm{sin}\left(2 \pi  (\frac{t} {\T_{ij}} + \boldsymbol{\theta}_{ij} )\right).
% \end{align}
% %
% where $\A_{ij}, \T_{ij}, \boldsymbol{\theta}_{ij}$ are the amplitude, period and phase shift for each control mode $i$ and sinusoidal function $j$. 
% %
% These quantities form the degrees of freedom (DOFs) for our controller, $\p = [\A \;\T  \;\boldsymbol{\theta}]^T \in \Rn{3 m_s \times m_t}$.




